Towards Tight Robust Coresets for $k$-Medians Clustering

This paper considers coresets for the robust $k$-medians problem with $m$ outliers, and new constructions in various metric spaces are obtained. Specifically, for metric spaces with a bounded VC or doubling dimension $d$, the coreset size is $O(m) + \tilde{O}(kd\varepsilon^{-2})$, which is optimal up to logarithmic factors. For Euclidean spaces, the coreset size is $O(m\varepsilon^{-1}) + \tilde{O}(\min\{k^{4/3}\varepsilon^{-2}, k\varepsilon^{-3}\})$, improving upon a recent result by Jiang and Lou (ICALP 2025). These results also extend to robust $(k,z)$-clustering, yielding, for VC and doubling dimension, a coreset size of $O(m) + \tilde{O}(kd\varepsilon^{-2z})$ with the optimal linear dependence on $m$. This extended result improves upon the earlier work of Huang et al. (SODA 2025). The techniques introduce novel dataset decompositions, enabling chaining arguments to be applied jointly across multiple components.

==> alg.tex <==

\section{Second Coreset Construction: Proof of Lemma~\ref{lemma_innergroup}}
\label{sec_innergroup}
Recall that $G$ is an $(r,k)$-instance and $G\subset B(A,r)$ for some $A=\{a_1,\cdots,a_k\}\in \binom{M}{k}$. Let $G_i=\{x\in G\mid i=\mathrm{argmin}_{j\in [k]} \dist(x,a_j)\}$ where ties in $\mathrm{argmin}$ are broken arbitrarily.

\begin{algorithm}[h]
    \caption{$\mathrm{Coreset}2(G,r,k,\eps, m)$}
    \label{alg_coreset2}
    \begin{algorithmic}[1]
        \REQUIRE An $(r,k)$-instance $G=G_1\cup\cdots\cup G_k$, parameters $\eps$, $m$, and a vanilla coreset oracle $\mathcal{B}$
        \ENSURE Coreset $D$
            \FOR{$i=1,\dots,k$}
                \STATE 
                $x_i\leftarrow$ an arbitrary point from $G_i$
                \STATE
                $H_i\leftarrow$ a subset of $\min(m,|G_i|)$ arbitrary points from $G_i$
                \STATE add $x_i$ with weight $w_D(x_i)=|H_i|$ to $D$
            \ENDFOR
            \STATE
            $H\leftarrow \bigcup_{i=1}^k H_i$
            \STATE
            $G_1\leftarrow G\setminus H$
            \STATE
                $D_1\leftarrow \mathcal{B}(G',\eps)$
            \STATE
                add $D_1$ to $D$
        \RETURN $D$
    \end{algorithmic}
\end{algorithm}



\eat{
\subsection{The algorithm}

We introduce some notation. As in most coreset algorithms, the first step is to find a constant factor approximation with centers $C^*=\{c_1^*,\dots,c_k^*\}$, so that $\cost[m](X,C^*)\leq O(1)\cdot \min_{C\in \binom{M}{k}}\cost[m](X,C)$. Let $L$ be the set of the $m+\lceil \eps^{-1} \rceil$ furthest points to $C^*$ in $X$ and define $Y=X\setminus L$. Let $r = \cost(Y,C^*)/|Y|$ denote the average cost of $Y$. For each $i\in[k]$, let $Y_i = \{y\in Y\mid i=\mathrm{argmin}_{i\in [k]} \dist(y,c_i^*)\}$ denote the set of inliers whose closest center is $c_i^*$, where ties in $\mathrm{argmin}$ are broken arbitrarily. Thus, $Y_1,\dots,Y_k$ form a partition of $Y$.

\paragraph{Balls and Rings} \emph{Balls} around $C^*$ are defined as $B_i=\{y\in Y\mid \dist(y,C^*)\leq 2^i\cdot\eps r\}$. We then define the \emph{rings} such that $R_0=B_0$ and $R_i=B_i\setminus B_{i-1}$ for $i=1,2,\dots,T$, where $T$ is the largest integer such that $R_T\neq\emptyset$. This implies that $T\leq \log \frac{|Y|}{\eps}$ and $R_0,\dots,R_T$ form a partition of $Y$. 

\paragraph{Decomposition of $X$} We decompose $X$ into three parts:
\[
    X = X_{\inn} \cup X_{\midd} \cup X_{\out},
\]
where
\begin{itemize}
    \item $X_{\out} = L$
    \item $X_{\midd} = \bigcup_{j=T-s+1}^T R_j$ for $s=\min\{\lceil \log (mk+1) \rceil,T\}$. These rings are also called the \emph{main rings}.
    \item $X_{\inn} = \bigcup_{j=0}^{T-s} R_j$. This set is also called the \emph{inner group}. It can be further decomposed into disjoint sets
    \[
        X_{\inn} = \bigcup_{i=1}^k G_i = \bigcup_{i=1}^k (H_i\cup G_i'),
    \]
    where $G_i := X_{\inn}\cap Y_i$ is the $i$-th cluster in $X_\inn$, the set $H_i\subseteq G_i$ is an arbitrary subset of size $\min\{m,|G_i|\}$ and $G_i' = G_i\setminus H_i$. We also denote $X_\inn' = \bigcup_{i=1}^k G_i'$ and $H = \bigcup_{i=1}^k H_i$, so $X_\inn = H\cup X_{\inn}'$.
\end{itemize}

% \paragraph{Inner Group} We collect the remaining rings and define them as the \emph{inner group}, denoted by $G=\bigcup_{i=0}^{T-s} R_i$. For each $i\in [k]$, let $G_i = G\cap Y_i$ and let $H_i\subset G_i$ be a subset consisting of $\min\{m,|G_i|\}$ arbitrarily chosen points from $G_i$. Define $G'_i=G_i\setminus H_i$, and set $H=\bigcup_{i\in [k]} H_i$ and $G'=\bigcup_{i\in [k]} G'_i$. Thus, $G=G'\cup H$. 

Let $\Delta = \max_i \diam(G_i)$.

\begin{lemma} \label{lemma_inner_dia}
It holds that $\Delta\leq \frac{\eps}{mk}\cdot \cost[m](X,C^*)$ for each $i\in [k]$.
\end{lemma}

\begin{proof}
Recall that $X=Y\cup L$ and $L=m+\lceil \eps^{-1}\rceil$, meaning that $\cost[m](X,C^*)$ aggregates at least $\lceil \eps^{-1}\rceil$ points outside the ball $B_T$. This implies that
\[
    \eps\cdot \cost[m](X,C^*)\geq  \frac{\cost[m](X,C^*)}{\lceil \eps^{-1}\rceil}\geq 2^T\cdot \eps r.
\]
Hence, for each $i\in [k]$,
\[
\diam(G_i) \leq 2\cdot 2^{T-s}\cdot \eps r\leq 2\cdot \frac{1}{2mk}\cdot 2^T\cdot \eps r\leq \frac{\eps}{mk}\cdot \cost[m](X,C^*). \qedhere
\]
\end{proof}

\paragraph{Coreset Construction Algorithm} Our coreset $D$ consists of three parts,
\[
    D = D_{\inn} \cup D_{\midd} \cup D_{\out},
\]
where
\begin{itemize}
    \item $D_{\out} = L$, where each point is associated with a unit weight.
    \item $D_{\midd} = \bigcup_{j=T-s+1}^T D_{j}$, where $D_{j}$ is an $(\eps,m,2^j\cdot \eps r)$-robust coreset of ring $R_j$. % These can be constructed using Algorithm~\ref{alg_coreset}.
    \item $D_{\inn} = D_H \cup D'$, where $D_0=\{(c_i^*,|H_i|)\mid i\in [k]\}$ and $D'$ is a vanilla $\eps$-coreset for $X_{\inn}'$.
% \item For each main ring $R_j$ ($T-s+1 \leq j\leq T$) we construct an $(\eps,m,2^j\cdot \eps r)$-robust coreset of $R_j$ using Algorithm~\ref{alg_coreset}. We add these robust coresets to $D$.  
% \item For the inner group $G$, we first add a $k$-point set $D_0=\{(c_i^*,|H_i|)\mid i\in [k]\}$ to $D$. Then we construct a vanilla $\eps$-coreset $D'$ of $G'$ and add $D'$ to $D$. By Theorem 1.2 of \cite{Cohen25}, $|D'|\leq \tilde{O}(kd\eps^{-2})$.
\end{itemize}
Each $D_j\subset D_{\midd}$ can be constructed using Algorithm~\ref{alg_coreset}. The vanilla coreset $D'$ can be constructed using Theorem 1.2 of \cite{Cohen25}, which guarantees that $|D'|\leq \tilde{O}(kd\eps^{-2})$.
}

\eat{
We first look at the coreset size. Clearly, Step 1 adds $O(m+\eps^{-1})$ points and Step 3 adds $\tilde{O}(kd\eps^{-2})$ many points. For Step 2, since $s=O(\log (mk))$, Theorem~\ref{thm_main} ensures that at most 
\[
    s\cdot \tilde{O}(kd\eps^{-2}) = \tilde{O}(kd\eps^{-2})\cdot \log(mk) 
    = O(m) + \tilde{O}(kd\eps^{-2})
\] 
points\footnote{Here we use the fact that $B\log A\leq B\log B+A$ for $A,B\geq 1$.} are added to $D$. Thus, the final coreset size is $O(m)+\tilde{O}(kd\eps^{-2})$.

By Fact~\ref{fact_merge} robust coresets are mergeable. Note that $D_\out$ and $D_\midd$ both have robust guarantees with respect to $X_\out$ and $X_\midd$, respectively. It remains to prove that $D_\inn$ is a robust coreset for $X_\inn$, that is, for every $C\in \binom{M}{k}$ and $t\in \{0,1,\dots,m\}$,
\begin{equation} \label{eq_inner}
\begin{aligned}
(1 - \eps) \cost[t](X_\inn,C) - K\eps \cost[m](X,C^*) 
&\leq 
\cost[t](D_\inn,C) \\
&\leq (1 + \eps) \cost[t](X_\inn,C) + K\eps \cost[m](X,C^*).
\end{aligned}
\end{equation}
for some absolute constant $K > 0$. We can then scale $\eps$ appropriately.
}

\begin{proof}[Proof of Lemma~\ref{lemma_innergroup}]

We prove that Algorithm~\ref{alg_coreset2} is the desired algorithm.

Let $D_H=\{(x_i,|H_i|)\mid i\in [k]\}$ denote the set of $k$ weighted points added into $D$ in the for loop. We prove that $D=D_H\cup D_1$ is an $(\eps,m,O(mkr))$-robust coreset of $G=H\cup G_1$.

We first argue, by losing an additive error of $O(mr)$, we can assume that the outliers in $\cost[t](H\cup G_1, C)$ are always chosen from $H$ and the outliers in $\cost[t](D_H\cup D_1, C)$ are always chosen from $D_H$. Specifically, let $J^\ast$ denote the set of the outlier points in $\cost[t](H\cup G_1, C)$ and $E^\ast$ the set of outlier points in $\cost[t](D_H\cup D_1, C)$. Let $J = (J^\ast\cap H)\cup J'$, where $J'\subseteq H\setminus J^\ast$ is an arbitrary subset such that $\abs{J'\cap H_i} = \abs{(J^\ast\setminus H)\cap G_i}$ for all $i\in [k]$. (This is always feasible since $\abs{G_i\cap J^\ast} \leq \min\{\abs{G_i},m\} = \abs{H_i}$ by our construction of $H_i$.)
Similarly, let $E = (E^\ast \cap D_H)\cup E'$, where $E'\subseteq D_H\setminus E^\ast$ satisfies that $\abs{E'} = \abs{E^\ast\setminus D_H}$. It follows that
\begin{align*}
    &\quad\ \abs{ \cost[t](D,C) - \cost[t](G,C) } \\
    &= \abs{ \cost(D\setminus E^\ast,C) - \cost(G\setminus J^\ast,C) } \\
    &\leq \abs{ \cost(D\setminus E,C) - \cost(G\setminus J,C) } + \abs{ \cost(E,C) - \cost(E^\ast,C) } + \abs{ \cost(J,C) - \cost(J^\ast,C) }\\
    &= \abs{ \cost(D\setminus E,C) - \cost(G\setminus J,C) } + \abs{ \cost(E',C) - \cost(E^\ast\setminus D_H,C) } \\
    &\hspace*{8cm} + \abs{ \cost(J',C) - \cost(J^\ast\setminus H,C) } \\
    &\leq \abs{ \cost(D\setminus E,C) - \cost(G\setminus J,C) } + 2mr + 2mr\\
    &= \abs{\cost(D_H\setminus E, C) - \cost(H\setminus J,C)} + \abs{\cost(D_1, C) - \cost(G_1,C)} + 4mr.
\end{align*}
We shall bound the first two terms separately.

For the first term, by the triangle inequality,
\[
    \abs{\cost(D_H\setminus E, C) - \cost(H\setminus J, C)}
    \leq \sum_{i\in [k]} \sum_{x\in H_i\setminus J} \dist(x,x_i)
    \leq 2mkr.
\]
where the last inequality follows from the fact that $\sum_i \abs{H_i} \leq mk$ due to the construction of $H$.

For the second term, since $D_1$ is a vanilla $\eps$-coreset of $G_1$, we have
\begin{align*}
    \abs{\cost(D_1, C) - \cost(G_1,C)} 
    &\leq \eps \cost(G_1, C) \\
    &\leq \eps \cost(G\setminus J, C) \\
    &\leq \eps \cost(G\setminus J^\ast, C) + \eps\abs{ \cost(J, C) - \cost(J^\ast, C) } \\
    &\leq \eps \cost(G\setminus J^\ast, C) + 2\eps m r \\
    &=\eps \cost[t](G,C) + 2\eps m r.
\end{align*}

%  By Lemma~\ref{lemma_inner_dia}, we know that $\diam(G_i)\leq \frac{\eps}{mk}\cdot \cost[m](X,C^*)$. Thus, by allowing an additive error of $2\frac{\eps}{k}\cdot \cost[m](X,C^*)$, 
%  we can assume the following: the outliers in $\cost[t](H\cup G', C)$ are always chosen from $H$ and the outliers in $\cost[t](D_0\cup D', C)$ are always chosen from $D_0$. Moreover, by the triangle inequality, we have that 
%  \begin{eqnarray*}
%  |\cost[t](D_0,C)-\cost[t](H,C)|&\leq& \sum_{i\in [k]}\sum_{x\in H_i} \dist(x,c_i^*)\\
%  &\leq & mk\cdot \frac{\eps}{mk}\cdot \cost[m](X,C^*)\\
%  &=& \eps \cdot \cost[m](X,C^*)
%  \end{eqnarray*}


% Since $D'$ is a vanilla $\eps$-coreset of $G'$ and no outliers have been removed from $D'$ or $G'$, we know that,
% \begin{align*}
% &\quad\ |\cost[t](D_0\cup D',C) - \cost[t](H\cup G',C)|\\
% &= |\cost[t](D_0,C)-\cost[t](H,C)|+|\cost(D',C)-\cost(G',C)| \\ %+2\eps\cdot\cost[m](X,C^*)\\
% &\leq \eps \cdot \cost[m](X,C^*)+\eps\cdot \cost(G',C) \\ %+2\eps \cdot \cost[m](X,C^*)\\
% &=\eps\cdot \cost(G',C) + \eps \cdot \cost[m](X,C^*) \\
% &\leq \eps\cdot \cost[t](H\cup G',C) + \eps \cdot \cost[m](X,C^*).
% \end{align*}

Therefore,
\begin{align*}
    \abs{ \cost[t](D,C) - \cost[t](G,C) }  
    &\leq \eps \cost^{(t)}(G, C) + (2mk+4m+2\eps m) r\\
    &\leq \eps\cost^{(t)}(G,C)+8mkr.
\end{align*}
%
and $D$ is an $(\eps,m,8mkr)$-robust coreset of $G$.
\end{proof}

==> kballs.tex <==

\section{Proof of Lemma \ref{lemma_mainring}: First Coreset for $(r,k)$-Instance}
\label{sec_mainring}
\eat{
Let $(M,\dist)$ denote a metric space where the ball range space has a VC dimension of $d$. For a point $x\in M$ and a radius $r>0$, let $B(x,r)=\{y\in M\mid \dist(x,y)\leq r\}$ denote the ball centered at $x$ with radius $r$. For a set $C=\{c_1,\dots,c_k\}\subset M$ and a radius $r>0$, let $B(C,r)=B(c_1,r)\cup\cdots\cup B(c_k,r)$. 
} 

Let $X=X_1\cup\cdots\cup X_k$ be an $(r,k)$-instance. We present an algorithm for constructing an $(\eps,m,\eps r \cdot |X|)$-robust coreset of $X$ for the $k$-median problem. We first introduce the notion of an $(r,k)$-\emph{regular instance}, which additionally requires that each $X_i$  contains a comparable number of points.

\begin{definition}[$(r,k)$-regular instance] A point set $X=X_1\cup\cdots\cup X_{k}\subset M$ is called an $(r,k)$-\emph{regular instance} if % $X_1,\cdots,X_{k}$ satisfy the following conditions:
\begin{enumerate}
    \item $\forall i,j\in [k]$, $i\neq j$, $X_i\cap X_j=\emptyset$;
    \item $\forall i,j\in [k], i\neq j$, $\abs{X_i} \leq 2\abs{X_j}$;
    \item $\forall i\in [k]$, $X_i\subseteq B(a_i,r)$ for some center $a_i\in M$.
\end{enumerate} 
\end{definition}


We let $X$ be an $(r,k_0)$-regular instance for some $k_0\leq k$ in the remainder of this section. Let $D$ be a weighted subset of $X$, we characterize a set of sufficient conditions for $D$ to form an $(\eps,m,\eps r\cdot |X|)$-robust coreset of $X$. We let $n:=|X|$ and $n_i:=|X_i|$ ($i\in [k_0]$) in the remainder of this section. Note that $\frac{n}{2k_0} \leq n_i \leq \frac{2n}{k_0}$ for all $i\in [k_0]$.




==> proof_subset.tex <==
\section{Proof of Lemma~\ref{lemma_subset}}
\label{sec_proof_subset}

Our proof employs a chaining argument developed in recent works \cite{fefferman2016testing,Cohen2022Towards,Cohen25}.  Recall that our instance is an $(r,k_0)$-regular instance, given by $X=X_1\cup\cdots\cup X_{k_0}$, where $X_i\subset B(a_i,r)$ for some $a_i\in M$. For every $x\in X$, let $\pi(x)$ denote the unique index $j\in [k_0]$ such that $x\in X_j$. Then $\dist(x,a_{\pi(x)})\leq r$.

Let $T=\lceil 1/\eps\rceil$. We define $A_0=[0,2r]$, and $A_i=(2^i r,2^{i+1}r]$ for each $i\in [T]$. Let $I_{i,C}=\{j\in [k_0]\mid \dist(a_j,C)\in A_i\}$ for each $i\in \{0,\dots,T\}$.

For every $i\in \{0,\dots,T\}$, $J\subseteq [k_0]$, $C\in \binom{C}{k}$, and every subset $S\subseteq X$, the distance vector $v_{i,J,C}^S:S\rightarrow \mathbb{R}_{\geq 0}$ is defined as
\[
v^S_{i,J,C}(x)=
\begin{cases}
    \dist(x,C), & \pi(x)\in J\cap I_{i,C} \\
    0, & \text{otherwise}.
\end{cases}
\]

Define the level-$i$ distance vector set as $V^S_{i}=\{v^S_{i,J,C}\mid J\subseteq [k_0],C\in \binom{M}{k}\}$. The following lemma establishes the relationship between subset approximation and $V_i^U$.

\begin{lemma}\label{lemma_relate} If for every $i\in \{0,\dots,T\}$, 
\begin{equation} \label{inq_chaining}
\sup_{J,C} \frac{n}{s}\cdot \abs*{ \frac{\sum_{x\in U} v^U_{i,J,C}(x)-\E \sum_{x\in U} v^U_{i,J,C}(x)}{(1+2^i|J_{i,C}|/k_0)\cdot nr} }
\leq \frac{\eps}{\log(1/\eps)},
\end{equation}
where $J_{i,C}=J\cap I_{i,C}$,
and event $\mathcal{E}$ (defined in \eqref{eq_event}) happens, then \eqref{inq_subset} holds. In other words, $U$ is an $\eps$-subset approximation of $X$.
\end{lemma}

\begin{proof}
Let $I_{far,C}=[k_0]\setminus \bigcup_{i=0}^T I_{i,C}$ and $J_{far,C}=J\cap I_{far,C}$. We observe that
$$
\cost(X_J,C)=\sum_{i=0}^T \cost(X_{J_{i,C}},C)+\cost(X_{J_{far,C}},C),
$$ and similarly
$$
\cost(U_J,C)=\sum_{i=0}^T \cost(U_{J_{i,C}},C)+\cost(U_{J_{far,C}},C).
$$
We shall show termwise approximations. First, we show that $$\cost(U_{J_{far,C}},C)\in (1\pm O(\eps))\cdot \cost(X_{J_{far,C}},C).$$ To see this, note that for each $x\in X_{J_{far,C}}$, $\dist(x,C)\geq \eps^{-1} r$. Thus for every $j\in J_{far,C}$, all points in $X_j$ have the same distance to $C$, up to a multiplicative $1+O(\eps)$ factor. When $\mathcal{E}$ happens, we have $w(U\cap X_j)\in (1\pm \eps)\cdot |X_j|$ for each $j\in [k_0]$, which implies $\cost(U_{J_{far,C}},C)\in (1\pm O(\eps))\cdot \cost(X_{J_{far,C}},C)$.

Now, for $i\in \{0,\dots,T\}$, observe that
\[
    \cost(U_{J_{i,C}},C)=\frac{n}{s}\cdot \sum_{x\in U} v^U_{i,J,C}(x)
    \quad\text{and}\quad
    \cost(X_{J_{i,C}},C)=\E\frac{n}{s}\cdot \sum_{x\in U} v^U_{i,J,C}(x).
\]
It follows from the assumption \eqref{inq_chaining} that
\[
\abs*{ \cost(U_{J_{i,C}},C)-\cost(X_{J_{i,C}},C) }\leq \frac{\eps}{\log \eps^{-1}}\cdot (1+2^i|J_{i,C}|/k_0)\cdot nr.
\]
Note that
\[
    \cost(X_{J_{i,C}},C)\geq |J_{i,C}|\cdot \frac{n}{2 k_0}\cdot 2^i r,
\]
thus
\[
    |\cost(U_{J_{i,C}},C)-\cost(X_{J_{i,C}},C)|\lesssim \frac{\eps}{\log \eps^{-1}}\cdot (\cost(X_{J_{i,C}},C)+nr)).
\]
%
Since there are $T+1=O(\log \eps^{-1})$ many $J_{i,C}$'s, by the triangle inequality,
we have that
$$
|\cost(U_J,C)-\cost(X_J,C)|\lesssim \eps \cost(X_J,C)+\eps n r.
$$
Rescaling $\eps$ completes the proof.
\end{proof}



A subset $N\subseteq V^S_i$ is called an $\alpha$-net of $V^S_i$ if for every $i,J,C$, there exists a vector $v\in N$ such that
\[
\begin{cases}
|v(x)-v^S_{i,J,C}(x)|\leq \alpha\cdot 2^{i+2}\cdot r & v^S_{i,J,C}(x)>0\\
0 & v^S_{i,J,C}(x)=0
\end{cases}
\]

The following lemma is essentially an adaption and extension of Lemma~5.3 of \cite{huang2023coresets} and Lemma~3.6 of \cite{Cohen25}. We include its proof for completeness.

\begin{lemma} \label{lemma_netsize}
For every $i\in \{0,\dots,T\}$, $\alpha\in (0,1)$ and every subset $S\subseteq X$ with $\abs{S}\geq 2$, there exists an $\alpha$-net $N^S_{\alpha,i}$ of $V^S_i$ such that
\[
\log \abs[big]{N^S_{\alpha,i}} \lesssim \alpha^{-1}d k\log k \cdot \log\abs{S}.
\]
Furthermore, if $\alpha\geq 2^{-i}$, it is possible to ensure that $N_{\alpha,i}^S$ consists of piecewise constant vectors. That is, every $v\in N_{\alpha,i}^S$ satisfies that $v(x)$ is a constant over all $x\in X_i$.
\end{lemma}

\begin{proof}

Let $\beta=\alpha 2^{i} r$. For a distance vector $v_{i,J,C}^S\in V_i^S$, we define its $\alpha$-rounding to be 
$$
\bar{v}_{i,J,C}^S(x) =  \left\lceil \frac{v_{i,J,C}^S(x)}{\beta} \right\rceil \cdot \beta.
$$
It is clear that $\bar{v}_{i,J,C}^S(x) \in \{0,\beta,\dots, \beta t\}$ for $t=\lceil 2/\alpha \rceil$.

We show that the collection of all $\alpha$-roundings
\[
    N_{\alpha,i}^S := \left\{\bar{v}_{i,J,C}^S\mid v_{i,J,C}^S\in V_i^S\right\}
\] 
is the desired net. 
The construction yields immediately that for every $x\in S$, $|\bar{v}_{i,J,C}^S(x)-v_{i,J,C}^S(x)|\leq \beta\leq \alpha\cdot 2^i\cdot r$ and $\bar{v}_{i,J,C}^S(x)=0$ if $v_{i,J,C}^S(x)=0$, which implies that $N_{\alpha,i}^S$ is indeed an $\alpha$-net of $V_i^S$. 

It remains to bound the size of $N_{\alpha,i}^S$. Consider each $u\in N_{\alpha,i}^S$, define for each $j\in \{0,\dots,t\}$ a ball $B_j^S=\{x\in S\mid u(x)\leq \beta \cdot j\}$. Since all coordinates of $u$ are fully determined by the sequence $B_0^S,\dots,B_t^S$, it suffices to bound the number of possible balls $B_j^S$. 
By construction, $B_0^S=(C\cap S)\cup (S\setminus X_{I_{i,C}})$, thus, the number of possible choices for $B_0^S$ is at most 
\[
    \binom{\abs{S}}{k}\cdot 2^k = |S|^{O(k)}.
\]
For $i\geq 1$, write $B_i^S$ as $B_i^S=(B(C, \beta\cdot i)\cap S)\cap X_{I_{i,C}}$. Since the VC dimension of $\mathrm{Balls}_k$ is at most $O(dk\log k)$~\cite{eisenstat2007vc}, the number of distinct choices for $B(C, \beta\cdot i)\cap S$ is
at most $|S|^{O(dk\log k)}$. Additionally, there are at most $2^k$ choices of $X_{I_{i,C}}$, leading to at most \[
    |S|^{O(dk\log k)}\cdot 2^k = |S|^{O(dk\log k)}
\]
distinct possibilities for each $B_i^S$, for each $i\in [t]$.
Consequently, the different number of combinations of $B_0^S,\dots,B_t^S$ can be bounded by 
\[
    |S|^{O(k)}\cdot (|S|^{O(dk\log k)})^{t}=|S|^{O(\alpha^{-1}dk\log k)},
\]
which is an upper bound on the size of $N_{\alpha,i}^S$.

When $\alpha\geq 2^{-i}$, we show that every $u\in N_{\alpha,i}^S$ can be made constant in each cluster. Define 
\[
\bar{u}(x)=
\begin{cases}
    \lceil \frac{\dist(a_{\pi(x)},C)}{\beta}\rceil\cdot \beta & u(x)>0\\
    0 & u(x)=0
\end{cases}
\]
Suppose $u\in N_{\alpha,i}^S$. Since $|u(x)-v_{i,J,C}^S(x)|\leq \beta$ for all $x\in S$, it follows that 
$|\bar{u}(x)-v_{i,J,C}^S(x)|\leq r + 2\beta\leq \alpha\cdot 2^{i+2}\cdot r$. 
If $v_{i,J,C}^S(x)=0$, we know that $u(x)=0$, then $\bar{u}(x)=0$ by construction.
Therefore, $\bar{N}_{\alpha,i}^S=\{\bar{u}\mid u\in N_{\alpha,i}^S\}$ is an $\alpha$-net of $V_{i,J,C}^S$ and every vector in  $\bar{N}_{\alpha,i}^S$ is a constant in each cluster. Furthermore,
\[
 \abs{\bar{N}_{\alpha,i}^S} \leq |N_{\alpha,i}^S|\leq |S|^{O(\alpha^{-1}dk\log k)}. \qedhere
\]
\end{proof}

It remains to prove the following lemma.

\begin{lemma} \label{lemma_chaining}
The bound \eqref{inq_chaining} holds for every $i\in \{0,\dots,T\}$ with probability at least $1-O\big(\frac{1}{\log \frac{k}{\eps}\cdot \log (mk)}\big)$.
\end{lemma}

\begin{proof}
It suffices to prove that for every $i\in\{0,\dots,T\}$,
\begin{eqnarray} \label{lemma_chaining_maininq}
    \E\sup_{J,C} \frac{1}{s}\cdot \abs*{ \frac{\sum_{x\in U} v^U_{i,J,C}(x)-\E \sum_{x\in U} v^U_{i,J,C}(x)}{(1+2^i|J_{i,C}|/k_0)\cdot r} }
    \lesssim \frac{\eps}{\log^2 \frac{1}{\eps}\cdot \log \frac{k}{\eps}\cdot \log mk},
\end{eqnarray}
then use Markov's inequality and take a union bound.

To ease the notation, let $\gamma_{i,J,C} = 1/(1+2^i|J_{i,C}|/k_0)$. The standard symmetrization trick gives that
\[
\E\sup_{J,C} \frac{\gamma_{i,J,C}}{rs}  \abs*{ \sum_{x\in U} v^U_{i,J,C}(x)-\E \sum_{x\in U} v^U_{i,J,C}(x) } 
\lesssim
\E_U \E_g \frac{1}{s} \sup_{J,C} \frac{\gamma_{i,J,C}}{r} \abs*{ \sum_{x\in U} g_x v^U_{i,J,C}(x) }
\]
%
For each $h\geq 0$, let $N_{2^{-h},i}^U$ be a ($2^{-h}$)-net of $V_i^U$ satisfying that
\[
    \log \abs[big]{N_{2^{-h},i}^U} \lesssim 2^h dk \log k \log s.
\]
which is possible by Lemma~\ref{lemma_netsize}. Furthermore, when $h = i$, one can ensure that $N_{2^{-i},i}^U$ consists of piecewise constant vectors.

By the net property, there exists a vector $b_{h,J,C}^U\in N_{2^{-h},i}^U$ such that
$$
|b_{h,J,C}^U(x)-v_{i,J,C}^U(x)|\leq 2^{i+2-h} r,\quad \forall x \in U.
$$ 
By writing $v_{i,J,C}^U(x)$ as the following telescoping sum
\[
v_{i,J,C}^U(x)=\sum_{h=i}^{\infty} \big(b_{h+1,J,C}^U(x)-b_{h,J,C}^U(x)\big)+b_{i,J,C}^U(x),
\]
we have
\begin{align*} 
&\quad\ \E_U \E_g \frac{1}{s} \sup_{J,C} \frac{\gamma_{i,J,C}}{r}\abs*{ \sum_{x\in U} g_x v^U_{i,J,C}(x) } \\
&\leq \E_U \frac{1}{s} \sum_{h=i}^\infty \E_g \sup_{J,C} \frac{\gamma_{i,J,C}}{r} \abs*{\sum_{x\in U} g_x (b_{h+1,J,C}^U(x)-b_{h,J,C}^U(x))} 
+ \E_U\frac{1}{s}\E_g \sup_{J,C} \frac{\gamma_{i,J,C}}{r} \abs*{\sum_{x\in U} g_x \cdot b_{i,J,C}^U(x)}
\end{align*}

We bound the two terms individually, starting with the first term. Consider the sum $\sum_{x\in U} g_x \big(b_{h+1,J,C}^U(x)-b_{h,J,C}^U(x)\big)$. 
Observe that $|b_{h+1,J,C}^U(x)-b_{h,J,C}^U(x)|\lesssim 2^{i-h} r$ and, by the construction of $V_i^U$, there are at most $\|U\cap X_{J_{i,C}} \|_0$ nonzero terms in the summation. Thus, the supremum in the first term is taken over $\abs[\big]{N^U_{2^{-h},i}}$ gaussians, each with a variance at most 
\[
    \gamma_{i,J,C}^2 \cdot 2^{2i-2h}\|U\cap X_{J_{i,C}}\|_0 
    \leq 2^{2i-2h} \sup_{J,C} \gamma_{i,J,C}^2 \|U\cap X_{J_{i,C}}\|_0.
\]
By the inequality for the maximum of Gaussians (Fact~\ref{fact_max_gauss}), we conclude that 
\begin{align*}
&\quad\ \E_U \frac{1}{s} \sum_{h=i}^\infty \E_g \sup_{J,C} \gamma_{i,J,C} \abs*{\sum_{x\in U} g_x (b_{h+1,J,C}^U(x)-b_{h,J,C}^U(x))}   \\
&\lesssim  \frac{1}{s}\sum_{h=i}^{\infty} 2^{i-h/2} \cdot \sqrt{dk\log k \log s}\cdot \E_U \sup_{J,C} \gamma_{i,J,C}\|U\cap X_{J_{i,C}}\|_0^{1/2}.
\end{align*}

% \begin{eqnarray*}
% &&\E_U\frac{1}{s}\sum_{h=i}^{\infty} \E_g\sup_{J,C}\bigg| \frac{\sum_{x\in U} g_x \cdot \big(b_h^U(x)-b_{h+1}^U(x)\big)}{(1+2^i|J_{i,C}|/k_0)\cdot r}
% \bigg|\\
% &\lesssim &
% \frac{1}{s}\sum_{h=i}^{\infty} 2^{i-h/2} \cdot \sqrt{dk\log k \log s}\cdot \E_U \sup_{J,C}\frac{\|U\cap X_{J_{i,C}}\|^{1/2}_0}{ 1+2^i|J_{i,C}|/k_0}
% \end{eqnarray*}

% We need to bound
% $$
% \E_U \sup_{J,C}\frac{\|U\cap X_{J_{i,C}}\|^{1/2}_0}{ 1+2^i|J_{i,C}|/k_0},
% $$
% and we have the following lemma.
We have the following lemma to bound the expected supremum on the right-hand side.
\begin{lemma} \label{lemma_chaining_var1}
It holds that $$
\E_U \sup_{J,C} \gamma_{i,J,C}\|U\cap X_{J_{i,C}}\|_0^{1/2} \lesssim \sqrt{\frac{s}{2^i}}
$$
\end{lemma}
\begin{proof}
Recall the event $\mathcal{E}$ defined in \eqref{eq_event}. When $\mathcal{E}$ happens, we have $\norm{U\cap X_\ell}_1 \in (1\pm \eps)\cdot |X_\ell|$ for every $\ell\in [k_0]$, which implies that $\frac{n}{s}\cdot \|U\cap X_{J_{i,C}}\|_0 \in (1\pm\eps) \cdot |X_{J_{i,C}}|$. Since $X$ is an $(r,k_0)$-regular instance, we know that $|X_{J_{i,C}}|\leq \frac{2|J_{i,C}|}{k_0}\cdot n$. It follows that $\|U\cap X_{J_{i,C}}\|_0\leq \frac{4|J_{i,C}|}{k_0}\cdot s$
and
%\begin{align*}
\[
\E_U \left[\sup_{J,C}\frac{\|U\cap X_{J_{i,C}}\|^{1/2}_0}{ 1+2^i|J_{i,C}|/k_0} \middle| \mathcal{E}\right]
\leq  \E \left[\sup_{J,C}\frac{\|U\cap X_{J_{i,C}}\|^{1/2}_0}{ 2\cdot (2^{i}|J_{i,C}|/k_0)^{1/2}} \middle| \mathcal{E} \right]\\
\lesssim \sqrt{\frac{s}{2^i}}
\]
%\end{align*}
where the first inequality is by $a^2+b^2\geq 2ab$ and the second inequality is by $\|U\cap X_{J_{i,C}}\|_0\leq \frac{4|J_{i,C}|}{k_0}\cdot s$.

On the other hand, it always holds that
\[
    \sup_{J,C}\frac{\|U\cap X_{J_{i,C}}\|^{1/2}_0}{ 1+2^i|J_{i,C}|/k_0} \leq k_0\sqrt{s}.
\]
Therefore,
\begin{align*}
\E_U \sup_{J,C} \gamma_{i,J,C}\|U\cap X_{J_{i,C}}\|_0^{1/2} &= \E_U \sup_{J,C}\frac{\|U\cap X_{J_{i,C}}\|^{1/2}_0}{ 1+2^i|J_{i,C}|/k_0}\\
&\leq \sqrt{\frac{s}{2^i}}\cdot \mathbb{P}(\mathcal{E}) + k_0\sqrt{s}\cdot \mathbb{P}(\bar{\mathcal{E}})\\
&\leq \sqrt{\frac{s}{2^i}} + k_0\sqrt{s}\cdot \frac{\eps}{sk}\\
&\lesssim \sqrt{\frac{s}{2^i}}.
\end{align*}
Here, the last inequality follows from the fact that $\frac{1}{2^{i/2}}\geq \frac{1}{2^i}\geq \frac{1}{2^T}\gtrsim \eps$.
\end{proof}

Hence, for the first term,
\begin{align*}
\E_U \E_g \frac{1}{s} \sup_{J,C} \gamma_{i,J,C}\abs*{ \sum_{x\in U} g_x v^U_{i,J,C}(x) }
&\lesssim  \frac{1}{\sqrt{s}}\sum_{h=i}^{\infty} 2^{i/2-h/2} \cdot \sqrt{dk\log k \log s} \\
&\lesssim  \sqrt{\frac{dk\log k \log s}{s}}\\
&\leq  \frac{\eps}{\log^2 \eps^{-1}\cdot \log \frac{k}{\eps}\cdot \log (mk)},
\end{align*}
provided that
\[
    s \gtrsim \frac{kd}{\eps^2} \cdot \log^{O(1)}(\frac{kd}{\eps})\cdot  \log^2 m.
\]

Next, we bound the second term
\[
\E_U\frac{1}{s}\E_g \sup_{J,C} \frac{\gamma_{i,J,C}}{r} \abs*{\sum_{x\in U} g_x \cdot b_{i,J,C}^U(x)}
 =
\E_U\frac{1}{s}\E_g \sup_{J,C} \abs*{ \frac{\sum_{x\in U} g_x \cdot b_{i,j,C}^U(x)}{(1+2^i|J_{i,C}|/k_0)\cdot r} }.
\]

If $J_{i,C}=\emptyset$, we have $b_{i,J,C}^U(x)=0$ for all $x\in U$ and the gaussian sum vanishes. Thus, it suffices to consider $J_{i,C}\neq\emptyset$ for the supremum. Then
\begin{align*}
\E_g \sup_{J,C} \abs*{ \frac{\sum_{x\in U} g_x \cdot b_{i,J,C}^U(x)}{(1+2^i|J_{i,C}|/k_0)\cdot r}
}
&\leq \E_g \sup_{J,C} \frac{\sum_{j\in J_{i,C}} \abs*{\sum_{x\in U\cap X_j} g_x \cdot b_{i,J,C}^U(x)}}{2^ir\cdot|J_{i,C}|/k_0} \\
&\leq \E_g\sup_{J,C}\max_{j\in J_{i,C}} \abs*{ \frac{\sum_{x\in U\cap X_j} g_x\cdot b_{i,J,C}^U(x)}{2^ir/k_0} }\\
&\leq \E_g \sup_{C}\max_{j\in I_{i,C}} \abs*{ \frac{\sum_{x\in U\cap X_j} g_x\cdot b_{i,J,C}^U(x)}{2^ir/k_0} }\\
&= \E_g \sup_{C}\max_{j\in I_{i,C}} \abs*{ \sum_{x\in U\cap X_j} g_x }\cdot \frac{k_0\cdot \norm{b_{i,J,C}^U}_{\ell^\infty(X_j)}}{2^ir}. 
\end{align*}
In the above, the third inequality is due to the definition that $J_{i,C}=J\cap I_{i,C}\subseteq I_{i,C}$, and the last equality the fact that $b_{i,J,C}^U(x)$ is a constant over each cluster.

Since $b_{i,J,C}^U(x)\leq v_{i,J,C}^U(x)+4r=\dist(x,C)+4r\lesssim 2^i r$, we can then bound
\begin{align*}
&\quad\ \E_U\frac{1}{s}\E_g \sup_{J,C} \abs*{ \frac{\sum_{x\in U} g_x \cdot b_{i,J,C}^U(x)}{(1+2^i|J_{i,C}|/k_0)\cdot r} } \\
&\leq \E_U\frac{1}{s}\E_g \sup_{C}\max_{j\in I_{i,C}} \abs*{ \sum_{x\in U\cap X_j} g_x 
}\cdot \frac{k_0\cdot \norm{b_{i,J,C}^U}_{\ell^\infty(X_j)}}{2^ir} \\
&\lesssim  \E_U\frac{k_0}{s}\cdot \E_g \sup_{C}\max_{j\in I_{i,C}}  \abs*{ \sum_{x\in U\cap X_j} g_x }\\
&\leq  \E_U\frac{k_0}{s}\cdot \E_g \max_{j\in [k_0]}  \abs*{ \sum_{x\in U\cap X_j} g_x }\\
&\lesssim \frac{k_0}{s}\cdot \sqrt{\log k_0} \cdot \E_U \max_{j\in [k_0]} \|U\cap X_j\|^{1/2}_0.
\end{align*}
where the last inequality follows from the observation that  $\max_{j\in [k_0]} \big|\sum_{x\in U\cap X_j} g_x \big|$ is the maximum of $k_0$ ganssians, each with a variance at most $\max_{j\in [k_0]} \|U\cap X_j\|_0$.

\begin{lemma} \label{lemma_chaining_var2}
$$
\E_U \max_{j\in [k_0]} \|U\cap X_j\|^{1/2}_0\lesssim \sqrt{\frac{s}{k_0}}.
$$
\end{lemma}

\begin{proof}
Identical to the proof of Lemma~\ref{lemma_chaining_var1}, we know that if $\mathcal{E}$ happens,  $\|U\cap X_j\|_0\leq \frac{4s}{k_0}$ for every $j\in [k_0]$. It follow from Lemma~\ref{lemma_event} that
\[
\E_U \max_{j\in [k_0]} \|U\cap X_j\|^{1/2}_0
\lesssim \sqrt{\frac{s}{k_0}}\cdot\mathbb{P}(\mathcal{E}) + \sqrt{s}\cdot \mathbb{P}(\bar{\mathcal{E}})
\lesssim \sqrt{\frac{s}{k_0}} + \sqrt{s}
\cdot \frac{\eps}{ks}
\lesssim \sqrt{\frac{s}{k_0}}. \qedhere
\]
\end{proof}

Therefore, the second term can be upper bounded as
\[
\E_U\frac{1}{s}\E_g \sup_{J,C} \abs*{ \frac{\sum_{x\in U} g_x \cdot b_{i,J,C}^U(x)}{(1+2^i|J_{i,C}|/k_0)\cdot r} }
\lesssim \sqrt{\frac{k_0\log k_0}{s}}
\leq \frac{\eps}{\log^2 \frac{1}{\eps}\cdot \log \frac{k}{\eps} \cdot \log (mk)},
\]
provided that 
\[
    s\gtrsim \frac{k}{\eps^2}\cdot \log^{O(1)} \frac{k}{\eps}\cdot \log^2 m.
\]
The bound \eqref{lemma_chaining_maininq} follows immediately and the proof is complete.
\end{proof}

The claim of Lemma~\ref{lemma_subset} follows immediately by combining Lemmata~\ref{lemma_event}, \ref{lemma_relate}, \ref{lemma_chaining}, and rescaling $\eps$.
